Dialogue-Based Relation Extraction

We present the first human-annotated dialogue-based relation extraction (RE) dataset DialogRE, aiming to support the prediction of relation(s) between two arguments that appear in a dialogue. We further offer DialogRE as a platform for studying cross-sentence RE as most facts span multiple sentences. We argue that speaker-related information plays a critical role in the proposed task, based on an analysis of similarities and differences between dialogue-based and traditional RE tasks. Considering the timeliness of communication in a dialogue, we design a new metric to evaluate the performance of RE methods in a conversational setting and investigate the performance of several representative RE methods on DialogRE. Experimental results demonstrate that a speaker-aware extension on the best-performing model leads to gains in both the standard and conversational evaluation settings. DialogRE is available at https://dataset.org/dialogre/.

==> History/1_introduction.tex <==
\section{Introduction}
%1. task of re, sentence->document (models & datasets), written->dialogue

Relation extraction (RE) is an important information extraction (IE) task that aims at extracting semantic relationships from text~\cite{miller2000novel,kambhatla2004combining,guodong2005exploring,surdeanu2012multi,min2012ensemble,min2013distant}. Most existing datasets~\cite{doddington2004automatic,roth2004linear,hendrickx2010semeval,riedel2010modeling,zhang2017position,han2018fewrel} and methods~\cite{socher2012semantic,zeng2014relation,zeng2015distant,dossantos2015classifying,lin2016neural,wu2017adversarial} for relation extraction focus on extracting relational facts from a sentence (\ie, sentence-level RE). Recently, researchers have begun to explore document-level RE, where relational facts to extract are not restricted to a single sentence~\cite{li2016biocreative,peng2017cross,quirk2017distant,yao2019docred,wang2019fine}. Texts in these studies are generally drawn from written documents such as news reports and Wikipedia. Relation extraction from oral texts, especially dialogues, by contrast, has not yet been studied systematically. 

%Relation extraction (RE) is a well-studied problem that aims at extracting semantic relationships from text

%2. importance: unique challenges in dialogue understanding; most information extraction tasks have been studied explicitly for dialogue); to advance research in re and facilitate dialogue understanding, we construct dialogRE; statistics;


Different from written documents, dialogues usually contain a considerable number of incomplete sentences, discursive markers, hesitation pauses, and rhetorical questions, and have more frequent use of colloquial language such as humors, slangs, ironies, or metaphors~\cite{perekhvalskaya2014mwan,chen2017robust,yang2019friendsqa}. These differences, together with the need for interpreting contents composed by multiple speakers in turns, constitute unique challenges for information extraction from dialogues. Therefore, a variety of IE tasks have been studied under dialogue-based settings such as dialogue-based coreference resolution and entity linking~\cite{chen2017robust,zhou2018they}). Following these studies, with the goal of advancing research in relation extraction and dialogue understanding, we present in this paper the first human-annotated dialogue-based relation extraction dataset DialogRE, which covers $36$ relation types (excluding no-relation) and contains $10,168$ relation instances annotated on $1,788$ dialogues.



%particularly, for dialogue-based re, in addition to difficulties at document-level RE, it further poses challenges: (1) dialogue structure (multi-turn, multi-speaker) (2) informal, common sense, evidence/trigger (3) short time relation (4) unsatisfying performance of underlying nlp components such as coreference resolution.


%relational facts

% Therefore, a variety of information extraction tasks have been studied under dialogue-based settings such as dialogue-based coreference resolution and entity linking~\cite{chen2017robust,zhou2018they}).
%Following recent studies on other information extraction tasks under dialogue-based settings such as dialogue-based coreference resolution and entity linking~\cite{chen2017robust,zhou2018they})

%Texts in these studies
%Texts in these sentence-level and document-level studies

%in multiple turns

%we present in this paper the first human-annotated dialogue-based relation extraction dataset DialogRE, accompanied by a study of methods and evaluation metrics for dialogue-based relation extraction. 

%we present in this paper a first study of dialogue-based relation extraction. 

%dataset DialogRE, accompanied by a study of methods and evaluation metrics for dialogue-based relation extraction.  %we present in this paper the first human-annotated dialogue-based relation extraction dataset DialogRE, accompanied by a study of methods and evaluation metrics for dialogue-based relation extraction. 

% present in this paper a study of dialogue-based relation extraction.

%with the goal of advancing research in relation extraction and dialogue understanding, we present the first human-annotated dialogue-based relation extraction dataset DialogRE. DialogRE covers $36$ relation types (excluding no-relation) and contains 10,168 relational facts annotated on 1,788 dialogues. 


%and have led to studies such as dialogue-based coreference resolution and entity linking~\cite{chen2017robust,zhou2018they}. 

%Different from written documents, dialogues usually contain a considerable number of incomplete sentences, discursive markers, hesitation pauses, and rhetorical questions, and have more frequent use of colloquial language such as humors, slangs, ironies, or metaphors\cite{perekhvalskaya2014mwan,chen2017robust,yang2019friendsqa}. These differences, together with the need for interpreting contents composed by multiple speakers in turns, pose unique challenges to information extraction and have led to information extraction research under dialogue-based settings such as dialogue-based coreference resolution and entity linking~\cite{chen2017robust,zhou2018they}. 


%We argue that dialogue-based relation extraction 
%Relation extraction from dialogues, however, has not yet been studied systematically.
%emerging studies
%Relation extraction, as a traditional information task, 
%However, there lacks a study on dialogue-based relation extraction.
%led to relevant studies
%have led to recent studies on dialogue-based information extraction such as dialogue-based coreference resolution and entity linking~\cite{chen2017robust,zhou2018they}.
%in recent years 
%to a growing interest in 
%the necessity of interpreting
%have led to recent studies on dialogue-based information extraction tasks such as dialogue-based coreference resolution and entity linking~\cite{chen2017robust,zhou2018they}.
%have led to relevant studies such as dialogue-based entity linking.
%Following recent progress in dialogue-based information extraction tasks
%Following recent progress in the development of
%, among which relation extraction from dialogues is one of the few that have not been studied systematically.
%, among which many have been recently studied such as named entity recognition, coreference resolution, and entity linking~\cite{chen2017robust,bowden2018slugnerds,zhou2018they}. %Researchers have A wide range of dialogue-based information extraction tasks have been recently studied, such as 

%However, relation extraction from dialogues, by contrast, has not yet been studied systematically. 

%a wide range of information extraction tasks
% various information extraction tasks

%pose unique challenges to information extraction tasks under dialogue-based settings.
%Dialogue understanding requires not only knowledge about sufficient knowledge of colloquial language that consists of humors, slang, ironies, or metaphors, but 





% 准确说明论文的创新点以及创新点的科学意义
% 恰当引用和说明眼球的起点和背景：前任的学术观点和贡献；目前该研究的进展情况
% 介绍重要结果，说明论文安排
% 承认确实size不大


%3.   explore and evaluate approaches under two settings



%4. what we find; we hope ....



%To advance research in relation extraction and dialogue understanding,

%formal informal % multiparty dialogue

%contributions: annotated dataset, comparison, metric, baselines, analysis

%https://www.aclweb.org/anthology/K17-1023.pdf
%Perhaps the most challenging aspect comes from colloquial writing that consists of ironies, metaphors, or rhetorical questions. Despite all the challenges, we believe that the output of this task will enhance inference on dialogue contexts by providing finer-grained information about individuals.

%https://www.aclweb.org/anthology/C18-1003.pdf
%Unlike most other entity linking tasks focusing on Wikification, this task is challenging because it is dialogue-based where the entities are general characters in the show

%https://www.aclweb.org/anthology/W19-5923.pdf
%Contextual understanding in dialogue is challenging because it needs to interpret contents composed by multiple speakers, and anticipate colloquial language filled with sarcasms, metaphors, humors, etc.

%(https://www.aclweb.org/anthology/W14-6509.pdf) Oral texts, especially dialogues, contain a large amount of incomplete sentences, hesitation pauses, discursive markers and loans from other languages, mainl


%and colloquial language that

%human-annotated
%We annotate 10,168 relations 1,788 dialogues, , and 36 
%DialogRE -- the first annotated dialogue-based relation extraction dataset. 
%We propose 
%We construct

%Following document-level RE, and 

%In comparison, oral texts, especially dialogues,
%extracting relational facts from 
%Texts in previous sentence-level and document-level RE studies are generally drawn from written documents such as news reports and Wikipedia,
%Texts in these studies are 
%Sentences/documents in these studies are 
%Sentences and documents in these previous studies
%Documents in these studies are mostly well-written texts such as news reports and Wikipedia,

%which are formal, accurate, and neutral.
%Recently, researchers have begun looking at inter-sentence relational facts, 
%Recently, researchers have begun to 
%the large number of inter-sentence relational facts 
%investigate document-level RE, where  

%the relational facts to extract are not restricted to  a single sentence
%Since inter-sentence relational facts
%Since there are a large number of relational facts expressed 
%sentence-level relation extraction methods cannot handle 
%a large number of relational facts are expressed in multiple sentences.

%Since sentence-level relation extraction
%~\cite{zelenko2003kernel,culotta2004dependency,kambhatla2004combining,guodong2005exploring,bunescu2005shortest,zhang2006exploring,socher2012semantic,zeng2014relation,zeng2015distant,xu2015classifying,dossantos2015classifying,lin2016neural,su2017global,luan2018multi}
%Most previous work on relation extraction mainly focuses on extracting relational facts from a single sentence~\cite{}. 
%Most existing datasets~\cite{doddington2004automatic,roth2004linear,hendrickx2010semeval,riedel2010modeling,zhang2017position,han2018fewrel} and methods~\cite{} for relation extraction focus on extracting relational facts from a single sentence. 
%intra-sentence relations
%Most previous work on relation extraction mainly focuses on extracting relational facts 



%validation: wang2008relation
%under several settings, including classification, trigger, and .



%\todo{===========K===========}



% 五个点的contributions

%differs from existing RE tasks in that

% though moderate size, xxxxx (自己先认了，省得被打)


spoken dialogue

human-to-human

challenges in dialogues:

compared to relations in formal corpus, relations that might remain a short time frequently appear in dialogues such as
per:positive\_impression and per:place\_of\_visited 

% 转折，

% 有两种setting: 旁观者（人，人，机），以及参与者 （人，机）

% 对话
% 1） 理解 （外部知识，以及对话者之间知道的事情，都可能隐藏）
% 2） 生成
% 3） 推理


%dialaogue上面 entity recognition, coreference resolution, entity linking一类的已经有了，to the best of our knowlege, the relations 还没做过

Relation extraction aims at extracting structured relational tuples from unstructured text~\cite{ji2005improving,jiang2007systematic}. The extracted tuples serve as critical input to a wide range of downstream tasks such as knowledge base population~\cite{McNamee2009,Ji2010,Ji2011,Surdeanu2014} and question answering~\cite{khot2017answering}. 




% zeng2014relation: relation classification
% xu2015classifying: classification
% relation extraction:kambhatla2004combining,guodong2005exploring,min2012ensemble,min2013distant,miller2000novel,surdeanu2012multi,wang2008relation,rahman2016graph
% ji2005improving




what makes dialogue-RE different/challenging:
1. dialogue: multi-turn multi-speaker
2. not merely sentence-level
3. predicate evidence
4. stronger coreference resolution is needed
5. unsatisfying performance of underlying nlp components such as pos/dependency parsing/ner



\hhide{
Baseline: 
1. raw sentence
RE: FINE-GRAINED:
1. RAW SENTENCE <E1>  </E1>  
2. entity, mrc, add diliminator, take segment (2 parts)
3. <>
datasets:
oft/base/large
}




%\todo{draw an overview figure...}
% --------------------------------------------------------------------------------------------------------------------%
%In this paper, we aim to investigate the effectiveness of pre-trained language models on relation extraction.



sentiment
comprehension
multi-turn




\hhide{
Specifically, (i) span-based machine reading comprehension has recently been adapted to relation extraction~\cite{nishida2018retrieve,levy2017zero}, and (ii) it has been shown that machine reading comprehension can benefit from pre-trained deep language models~\cite{radfordimproving,bert2018}. Inspired by these efforts, we propose two directions of study: (a) combine (i) and (ii) (\ie, adapt machine reading comprehension (extractive or non-extractive) improved by pre-trained language models to relation extraction and validation); and (b) directly adapt a pre-trained language model to relation extraction and validation following the methodology of (ii). We believe that the proposed method has the following potential contributions:
\begin{itemize}
    \item Contextual information is useful to facilitate the detection of both explicit and implicit relations~\cite{petroni2015core,sorokin2017context}. Compared to the utilization of lexical or syntactic features derived from the context in previous work, exploiting a language model is a natural choice since it makes use of full contextual information in an input sequence.
    \item Pre-trained deep language models leverage rich general world knowledge from a large-scale corpus during pre-training. While previous work has exploited structured knowledge such as high-quality knowledge bases and lexicons cleaned by human annotators, we hypothesize that incorporating general world knowledge that implicitly exists in a pre-trained language model can boost the performance of relation extraction and validation.
\end{itemize}
}

%It consists of 185k claims generated by altering sentences extracted from Wikipedia and subsequently verified without knowledge of the sentence they were derived from. The claims are classified as ``supported'', ``refuted'' or ``not enough info''.
%\textbf{Semeval 2019 Task 8}\footnote{http://alt.qcri.org/semeval2019/}


















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%HISTORY%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hhide{



https://arxiv.org/pdf/1707.01075.pdf

http://www.aclweb.org/anthology/W14-2508

http://cistern.cis.lmu.de/SFbenchmark/

Heike Adel, Benjamin Roth, and Hinrich Schutze. ¨ 2016. Comparing convolutional neural networks to traditional models for slot filling. In Proc. NAACL2016

http://aclweb.org/anthology/W18-5517


-------------------------------------------------------

\textbf{Existing}

* simple question generation + extractive machine comprehension models~\cite{levy2017zero,nishida2018retrieve}
  
  ** question generation: template~\cite{levy2017zero} or question generation models~\cite{duan2017question,wang2017joint}
   


\noindent-------------------------------------------------------

\textbf{OURS}

* use slot filling, slot filling validation, and fever as case studies to evaluate the effectiveness of our approach

* change to the multiple-choice settings

* question generation baseline: use patterns from RPI, NYU, and BUPT

* question generation based on descriptions in the guideline

* make sure more than 80-85\% answers appear in the distractors (guarantee the recall first)

* consider distance constraints and entity type constraints when we design/generate answer options (candidates)
%* (distance constraints, wo wang le zhe tiao zai shuo sha le) 

* follow the original slot filling setting: provide evidence sentences $\to$ useful in an adversarial setting~\cite{jia2017adversarial,min2018efficient}


\noindent-------------------------------------------------------
}

==> History/5_relatedwork.tex <==
\section{Related Work}

%\subsection{Sentence-Level Relation Extraction}
\subsection{Datasets for Relation Extraction}

\begin{table*}[]
\centering
\small
\begin{tabular}{llllll}
\toprule
\bf Task                 & \bf style of doc   & \bf \# of doc & \bf source of doc & \bf \# of rel & \bf \# of instances$^\star$\\
\midrule
\multicolumn{6}{c}{----- distant supervision -----}                                       \\
\midrule
DocRED~\cite{yao2019docred}      & written            &  101,873   &  Wikipedia  & 96         & 1,508,320               \\
%DialogRE (this work)              & oral             &     &  Friends                    &  36        & 8,068                  \\
\midrule
\multicolumn{6}{c}{----- human annotated -----}                                                                           \\
\midrule
BC5CDR~\cite{li2016biocreative}   & written             &  1,500  &  PubMed                     &  1         & 3,116                  \\
DocRED~\cite{yao2019docred}       & written             & 5,053   &  Wikipedia                  &  96        & 63,427                  \\
DialogRE (this work)              & oral                &  1,788  &  Friends                    &  36        & 8,068                  \\
\bottomrule
\end{tabular}
\caption{\label{tab:related}Statistics of document-level relation extraction datasets ($\star$: not include no-relation instances).}
\end{table*}



Much of the early work focuses on constructing datasets for sentence-level relation extraction, the task of which is to extract relations between a pair of entity mentions in the same sentence. Representative datasets include ACE'04 and ACE'05 from the Automatic Content Extraction ({ACE}) program~\cite{doddington2004automatic}, CoNLL'04 corpus of \citet{roth2004linear}, SemEval-2010 Task 8~\cite{hendrickx2010semeval}, and NYT'10 corpus developed by \citet{riedel2010modeling}. In recent years, while more sentence-level relation extraction datasets are released~\cite{zhang2017position,han2018fewrel}, there is a growing interest in constructing document-level relation extraction datasets~\cite{quirk2016distant,li2016biocreative,peng2017cross,yao2019docred}. Documents in these datasets have generally been drawn from written texts. In contrast, DialogRE is the first annotated document-level relation extraction dataset whose documents are dialogues. We compare them in Table~\ref{tab:related}.




% such as news reports and Wikipedia


%formal written texts
%there is a growing interest in constructing
%We divide relation extraction datasets into 
%Much of the early work focuses on extracting relations between a pair of entity mentions in the same sentence. Representative datasets include ACE'04 and ACE'05 from the Automatic Content Extraction ({ACE}) program~\cite{doddington2004automatic}, CoNLL'04 corpus of \citet{roth2004linear}, SemEval-2010 Task 8~\cite{hendrickx2010semeval}, and NYT'10 corpus developed by \citet{riedel2010modeling}. 

%constructing manually annotated datasets

%Researchers construct manually annotated datasets, 

%Much of the early work focuses on relation extraction at the sentence level. 

%The Automatic Content Extraction ({ACE}) Program~\cite{doddington2004automatic}
%ACE04 ACE 05

%CoNLL04~\cite{roth2004linear}

%NYT~\cite{riedel2010modeling}

%SemEval~\cite{hendrickx2010semeval}


%\subsection{Document-Level Relation Extraction}


%document-level relation extraction
%~\cite{quirk2016distant,peng2017cross}: distant supervision, no human involvement

%BC5CDR~\cite{li2016biocreative}: bio-medical, 1500 documents, human annotated

%Existing datasets
%for document-level RE either only have a small number of manually-annotated relations and entities, or exhibit noisy annotations from distant supervision before DocRED~\cite{yao2019docred}, the first large-scale human annotated document-level RE dataset. However, the source of documents are all from Wikipedia articles, which are formal and well-written. 

%To the best of our knowledge, this is the first dialogue-level relation extraction dataset.


\subsection{Dialogue Understanding} %Dialogue-Based Information Extraction
%\subsection{Dialogue-Based Machine Reading Comprehension}

As there are unique challenges in dialogue understanding compared to understanding other forms of language use, there is a research trend towards studying NLP tasks explicitly under dialogue-based settings, such as named entity recognition~\cite{bowden2018slugnerds}, coreference resolution~\cite{chen2017robust,zhou2018they}, entity linking~\cite{chen2017robust,zhou2018they}, question answering~\cite{yang2019friendsqa}, and reading comprehension~\cite{sun-etal-2019-dream}. Among traditional information extraction tasks~\cite{ralph2019twenty}, relation extraction is one of the few that have not been studied before in the literature within a dialogue-based setting. %relation extraction is the only task that has not been studied before in the literature within a dialogue-based setting.

%https://www.aclweb.org/anthology/N15-1086.pdf
% dialogue目的不一样，为了构建KB, 对话引导方题目有点偏multiple-choice science QA, instead, parties are humans in our setting
% 跟peter clark研究兴趣重合的还真多。。。


%As there are unique challenges in dialogue understanding compared to understanding other forms of language use, a wide range of NLP tasks is explicitly studied under dialogue-based settings such as named entity recognition~\cite{bowden2018slugnerds}, coreference resolution~\cite{chen2017robust,zhou2018they}, entity linking~\cite{chen2017robust,zhou2018they}, question answering~\cite{yang2019friendsqa}, and reading comprehension~\cite{sundream2018}.

%
%within dialogue-based settings.
%. %natural language understanding  %with dialogue-based  %dialogue-based versions of %there is a research trend towards 

%As understanding dialogues 
%unique challenge
%understanding written language
%other genres of texts, 
%compared to written text, 


\subsection{Approaches for Relation Extraction}

Early studies in relation extraction mainly use hand-crafted features~\cite{kambhatla2004combining,guodong2005exploring} and kernel methods~\cite{zelenko2003kernel,culotta2004dependency,bunescu2005shortest,zhang2006exploring}. In recent years, considerable success has been achieved by employing neural models~\cite{zeng2015distant,lin2016neural,su2017global}, in which the representation of an input sequence usually comes from shallow neural networks over pre-trained word embeddings and character embeddings~\cite{xu2015classifying,zeng2015distant,lin2016neural}. Researchers have also recently applied deep contextualized word representations such as the ELMo~\cite{Peters:2018} as additional input features to boost the performance of relation extraction~\cite{luan2018multi}. Very recently, we have seen research efforts move from leveraging word representation as features to directly fine-tuning pre-trained deep language models~\cite{radfordimproving,bert2018} on relation extraction tasks~\cite{alt2019improving,wang2019fine}.

%move from using deep word representations as features 
%the success of fine-tuning pre-trained deep language models on many downstream NLP tasks~\cite{radfordimproving,bert2018} motivates a move to fine-tuning pre-trained deep language models.
%Very recently, we have seen research efforts move from deep word representations~\cite{Peters:2018} to deep language models~\cite{radfordimproving,bert2018}. In particular, with the help of deep language models pre-trained on large-scale corpora such as the BooksCorpus~\cite{zhu2015aligning,radfordimproving,bert2018} and Wikipedia~\cite{bert2018}, and further fine-tuned on a supervised target task, new state-of-the-art has been achieved in a range of natural language understanding tasks including named entity recognition, sentiment analysis, textual entailment, question answering, and machine reading comprehension. To the best of our knowledge, such pre-trained high-capacity language models have not yet been successfully applied to relation extraction, which usually requires a deeper understanding of the relations between entities or concepts. It is still an open problem whether or not relation extraction can benefit from pre-trained language models that leverage rich external linguistic knowledge.

%Whether or not pre-trained deep language models that leverage rich linguistic knowledge over large-scale corpora can bring improved performance on both relation extraction and validation is still an open problem.


\iffalse

%https://www.aclweb.org/anthology/P19-1549
%这篇不算re吧?
%我咋看着像generation
%response generation

extractive (unanswerable): FriendsQA
multiple-choice: DREAM


~\cite{levy2017zero} formulate re as a machine reading comprehension problem
aligning each Wikidata relational entity pair (e, a) with the corresponding Wikipedia
article D for the entity e, under the reasonable assumption that the relation can be derived from the
article's text. Still, the document are formal documents from Wikipedia.


% transfer
MultiQA: An Empirical Investigation of Generalization and Transfer in Reading Comprehension


% emotions
MELD: A Multimodal Multi-Party Dataset for Emotion Recognition in Conversations


% vsually grounded
The PhotoBook Dataset: Building Common Ground through Visually-Grounded Dialogue
Janosch Haber, Tim Baumgärtner, Ece Takmaz, Lieke Gelderloos, Elia Bruni and Raquel Fernández



% check the following
Episodic Memory Reader: Learning What to Remember for Question Answering from Streaming Data



human to machine
%https://www.aclweb.org/anthology/W11-2008



Learning Knowledge Graphs for Question Answering through Conversational Dialog
% https://www.aclweb.org/anthology/N15-1086


Using Syntactic and Semantic based Relations for Dialogue Act Recognition
%https://www.aclweb.org/anthology/C10-2065



OpenKI: Integrating Open Information Extraction and Knowledge Bases with Relation Inference". In NAACL 2019
movies: distant supervision




Unifying Question Answering and Text Classification via Span Extraction
https://arxiv.org/pdf/1904.09286

1. pattern-based

2. supervised methods/distant supervision/rnn

3. pre-trained models (as features or fine-tuned)

argument mining
http://aclweb.org/anthology/W15-4631

Extracting Networks of People and Places from Literary Texts
http://aclweb.org/anthology/Y12-1022
SOCIAL NETWORK FROM LITERARY FICTION
http://www.aclweb.org/anthology/P10-1015


involve human
http://aclweb.org/anthology/N15-1086


summarization via unsupervised re in dialogues (Lu Wang and CTC)
http://www.aclweb.org/anthology/W12-1642


for dialogue MRC?

%difference summarized here or use a table?

cross-lingual (english and chinese)

entity linking and coreference resolution in dialogues
http://www.aclweb.org/anthology/K17-1023

http://aclweb.org/anthology/C18-1003

http://aclweb.org/anthology/S18-1007

http://www.aclweb.org/anthology/W16-3612

tac:
https://nlp.stanford.edu/pubs/zhang2017tacred.pdf

%\subsection{Dialogue-Based Machine Reading Comprehension}
\fi



\hhide{
% todo Dian
Traditional Information Extraction: relationships are manually annotated, and belongs to pre-determined type. (dialogre)

Open Information Extraction: relationships are manually annotated, but don't have any specific type. (future work, perhaps mention this one, and how to automatically segment dialogues from transcripts)

Distantly Supervised: relationships are annotated by appying some Distant Supervision technique and are pre-determined. (check dongxu's work)


EMNLP 2019
Knowledgenet:
https://www.aclweb.org/anthology/D19-1069.pdf
cross-sentence KBP, Table 1
what's the difference of document-based and cross-sentence?
% 说document的时候有点vague
}
